Revisiting MITL to Fix Decision Procedures

Metric Interval Temporal Logic (MITL) is a well studied real-time, temporal logic that has decidable satisfiability and model checking problems. The decision procedures for MITL rely on the automata theoretic approach, where logic formulas are translated into equivalent timed automata. Since timed automata are not closed under complementation, decision procedures for MITL first convert a formula into negated normal form before translating to a timed automaton. We show that, unfortunately, these 20-year-old procedures are incorrect, because they rely on an incorrect semantics of the R operator. We present the right semantics of R and give new, correct decision procedures for MITL. We show that both satisfiability and model checking for MITL are EXPSPACE-complete, as was previously claimed. We also identify a fragment of MITL that we call MITL_{WI} that is richer than MITL_{0,\infty}, for which we show that both satisfiability and model checking are PSPACE-complete. Many of our results have been formally proved in PVS.

==> part-2vars.tex <==
\section{Two Variables Are Not Enough}\label{sec:2vars}
In this section, let $p$ and $q$ be two distinct atomic propositions, and let $\II$ be an arbitrary non-negative interval that is neither empty 
nor singleton.
% 
The main result of this section is that, 
	under fairly general syntactical constraints including using only two variables, 
	even if we redefine semantics of \ReleaseOp\ operator, separately, for every possible $\Release{\varphi_1}{\varphi_2}[\JJ]$, 
	it will be still impossible to make $\neg\Paren{\Until{p}{q}[\II]}$ and $\Release{\neg p}{\neg q}[\II]$ equivalent.
This remains true, even if we restrict our attention to signals that change their values finitely many times throughout the entire time domain.	
%
First, we use \Ex~\ref{ex:2vars} to show that the current semantics of $\ReleaseOp$ operator, as specified in \aref{def:mtl-sem}, makes 
$\neg\Paren*{\Until{p}{q}[\II]}$ and $\Release{\neg p}{\neg q}[\II]$ inequivalent.
Note that this example alone, shows that the current decision procedures for satisfiability and model checking \MITL\ and \MITLzi, as defined 
in~\cite{96-MITL}, are in fact flawed.
%
\Thm~\ref{thm:2vars} states our main results of this section and the rest is devoted to proving it.

\vskip\baselineskip
\noindent
\begin{minipage}{0.65\textwidth}
\begin{example}\label{ex:2vars}
Let $c\oftype\Open{\II}$ be an arbitrary point, and define $\Sgn$ to be the signal
	$\Paren*{\Braket{0,c},\Brace{p}},\allowbreak
	 \Paren*{\Paren{c,\infty},\Brace{q}}$.
Clearly, $\Sgn\ONSat\Until{p}{q}[\II]$ and hence $\Sgn\OSat\neg\Paren*{\Until{p}{q}[\II]}$ are true.
On the other hand, 
	$\neg q$ is not true throughout $\II$ and whenever $\neg p$ is true, $\neg q$ is false.
	Therefore, $\Sgn\ONSat\Release{\neg p}{\neg q}[\II]$, which makes $\ReleaseOp$ \emph{not} dual of $\UntilOp$.
\end{example}
\end{minipage}
\hfill
\begin{minipage}{0.32\textwidth}
\vskip-1.75\baselineskip
\begin{figure}[H]
\scalebox{0.865}{\input{./fig-2vars-sig}}
\vskip-\baselineskip
\caption{Signal \Sgn}\label{fig:2vars-sig}
\end{figure}
\end{minipage}


\begin{theorem}\label{thm:2vars}
For every triple $\varphi_1$, $\varphi_2$, and $\JJ$, 
	let semantics of $\Release{\varphi_1}{\varphi_2}[\JJ]$ be redefined using some formula 
	$\Phi_{\varphi_1,\varphi_2,\JJ}\Paren*{\Sgn}$ in the following form.
Then formula $\neg\Paren*{\Until{p}{q}[\II]}$, 
	as defined in \Def~\ref{def:mtl-sem}, won't be equivalent to $\Release{\neg p}{\neg q}[\II]$, even for signals that change their values at most $4$ times
	throughout the entire time domain.
\[
  \bigwedge_{i\oftype\Brace{1,\ldots,n}}\bigvee_{j\oftype\Brace{1,\ldots,i_n}}
  \exists t_1\oftype\Real\SuchThat\forall t_2\oftype\Real\WeHave\phi_{i,j}\Paren*{\Sgn,t_1,t_2}
\]
$n\oftype\Nat$ is arbitrary, 
$i_n\oftype\Nat$ only depends on $i$, and
formula $\phi_{i,j}$ is defined using the following \BNF\ notation~\footnote{%
  $n$, $i_n$, and $\phi_{i,j}$ are all defined separately for each combination of $\varphi_1$, $\varphi_2$, and $\JJ$.
  We do not put these parameters as index only to make the notation simpler.}:
\[
	\phi  ::=
	\top																	\filter
	\neg\phi															\filter
	\phi\vee\phi													\filter
	\alpha_1 t_1+\alpha_2 t_2\bowtie\beta	\filter
	\Sgn^{t_u}\OSat\varphi_v							
\] 
where 
	$\alpha_1,\alpha_2,\beta\oftype\Real$ are arbitrary constants,
	$\bowtie\oftype\Brace{<,\leq,>,\geq}$ is an arbitrary relation symbol, and
	$u,v\oftype\Brace{1,2}$.
We call 
	constraints of the form $\alpha_1 t_1+\alpha_2 t_2\bowtie\beta$	\emph{domain} constraints and 
	constraints of the form $\Sgn^{t_u}\OSat\varphi_v$								\emph{signal} constraints~\footnote{%
Strictly speaking, instead of $\Sgn^{t_u}\OSat\varphi_v$, we should define and use a new $\Sat$ operator in the syntax of $\phi_{i,j}$ that uses the 
new definitions for $\ReleaseOp$ operator, and uses \Def~\ref{def:mtl-sem} for every other operator. But since, in this theorem we are only interested in the case
$\varphi_1$ and $\varphi_2$ do \emph{not} contain temporal operators, the current simpler syntax will be equivalent and hence enough for our 
purpose.}.
\end{theorem}
 
Note that the following restrictions over the syntax of $\Phi_{\varphi_1,\varphi_2,\JJ}$ do not reduce its expressivity:
\begin{inparaenum}
\item $\Phi_{\varphi_1,\varphi_2,\JJ}$ must be given in \CNF,
\item there is no $\vee$ or $\wedge$ connectives between $\exists t_1\oftype\Real$ and $\forall t_2\oftype\Real$, and
\item only $\varphi_1$ and $\varphi_2$ are allowed in the right hand side of $\OSat$ operator (not their boolean combinations).
\end{inparaenum}
The most important restrictions are 
\begin{inparaenum}
\item $\Phi_{\varphi_1,\varphi_2,\JJ}$ can only have linear domain constraints, and
\item $\Sgn$ can be shifted by only $t_1$ or $t_2$ and not any combination of them.
\end{inparaenum}
Finally, \wLOG, we assume whenever $\Sgn^{t_1}$ and $\Sgn^{t_2}$ are used, values of $t_1$ and $t_2$ are guaranteed to be non-negative.


For the purpose of contradiction, 
	let $\Phi_{\neg p,\neg q,\II}$ makes $\neg\Paren*{\Until{p}{q}[\II]}$ and $\Release{\neg p}{\neg q}[\II]$ equivalent, 
	at least for signals that change their values at most $4$ times throughout the entire time domain.
Thus, for any such  signal $\Sgn$, we have $\Sgn\OSat\neg\Paren*{\Until{p}{q}[\II]}$ \iFF\ $\Sgn\NSat\Release{\neg p}{\neg q}[\II]$.
%Proof has multiple steps and are explained in \Sec~\ref{sec:smpl} through \Sec~\ref{sec:contradiction}.
Steps of the proof are explained in \Sec~\ref{sec:smpl} through \Sec~\ref{sec:contradiction}.

%%---------------------------------------------------------------------------------------------------------------------------------------------------
%%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Simplifications}\label{sec:smpl}
Applying required transformations, \wLOG, assume the following conditions about $\Phi_{\neg p,\neg q,\II}$.
\begin{myenums}
\item \label{smpl:top-free}
			It is free of $\top$ operator. 
\item \label{smpl:neg-free}
			Operator $\neg$ only appears in front of $p$ and $q$.
			This is always possible since $\Brace{<,\leq,>,\geq}$ is closed under negation and $\neg\Paren{\Sgn^t\OSat\varphi}$ is, by definition, 
			equivalent to $\Sgn^t\OSat\neg\varphi$.
			Note that after this step, $\phi_{i,j}$ may contain $\wedge$ operator.
\item \label{smpl:cnf}
			Every $\phi_{i,j}$ is in \CNF.
\item \label{smpl:S}
			Every clause in $\phi_{i,j}$, has at most 
			one signal constraint of the form $\Sgn^{t_1}\OSat\psi_1$ and 
			one signal constraint of the form $\Sgn^{t_2}\OSat\psi_2$ where
			$\psi_1$ and $\psi_2$ are boolean combinations of $p$ and $q$.
\item \label{smpl:P}
			For an arbitrary clause $\phi_{i,j,k}$ in $\phi_{i,j}$, 
				let $S$ and $P$ be, respectively, the set of signal and \emph{negated} domain constraints in $\phi_{i,j,k}$.
			$\phi_{i,j,k}$ is equivalent to $\Paren*{\bigwedge_{\theta\oftype P}\theta}\Implies\Paren*{\bigvee_{s\oftype S}s}$.
			The left hand side of this implication defines a 2-dimensional convex polyhedron using variables $t_1$ and $t_2$.

			For the rest of the proof, \wLOG, we assume every clause in every $\phi_{i,j}$ is of the form $P\Implies S$, where $P$ is a polyhedron over 
      $t_1$ and $t_2$, and $S$ is a disjunction of $0$, $1$, or $2$ signal constraints.
			For any polyhedron $P$, we define $\Sem{P}\defEQ\Brace{\Paren{t_1,t_2}\filter P(t_1,t_2)}$ to be the set of points in $P$.
      Also, $\Closure{\Sem{P}}$ is defined to be the closure of $\Sem{P}$.
			Finally, let $\PP$ be the set of all polyhedra used in $\Phi_{\neg p,\neg q,\II}$.
\item \label{smpl:disjoint}
			Since for any three polyhedra $P_1$, $P_2$, and $P$ over variables $t_1$ and $t_2$, and a set of signal constraints $S$,
			if $\Sem{P_1}\cup\Sem{P_2}=\Sem{P}$ then $\Paren{P_1\Implies S}\wedge\Paren{P_2\Implies S}$ is equivalent with $P\Implies S$,
			assume $\forall P_1,P_2\oftype\PP\WeHave \Sem{P_1}=\Sem{P_2} \vee \Sem{P_1}\cap\Sem{P_2}=\emptyset$.
\end{myenums}


\setlength\abovecaptionskip{0pt}%
\setlength\belowcaptionskip{0pt}%
\begin{wrapfigure}{r}{30mm}%
\raggedleft%
\vspace{-1.2\baselineskip}%
\includegraphics[width=30mm]{./fig-conditional.pdf}%
\caption{}\label{fig:conditional}%
\end{wrapfigure}%
\setlength\abovecaptionskip{\baselineskip}%
\setlength\belowcaptionskip{\baselineskip}%
%
\Fig~\ref{fig:conditional} shows geometrical interpretation of polyhedral representation of constraints in $\Phi_{\neg p,\neg q,\II}$.
Let $\phi_{i,j,k}$ be a clause that is specified by $P\Implies S$.
An arbitrary horizontal line $L$, may or may not have intersection with $P$.
Either way, $L$ {\em witnesses} $\exists t_1\SuchThat\forall t_2\WeHave\phi_{i,j,k}$ \iFF\ for all points in this possibly empty intersection, $S$ is satisfied.
Every $\phi_{i,j}$ is a set of constraints of the form $P\Implies S$. Therefore,
$L$ {\em witnesses} $\exists t_1\SuchThat\forall t_2\WeHave\phi_{i,j}$ \iFF\ $L$ witnesses all clauses in $\phi_{i,j}$.
Furthermore, $\exists t_1\SuchThat\forall t_2\WeHave\phi_{i,j}$ is true \iFF\ there is a horizontal line $L$ that witnesses it.

%%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Defining $\delta$ and $r$}\label{sec:consts}
For any $P\oftype\PP$ define $V_P$ to be the set of vertices of $P$, and
														 $L_P$ to be the set of points on \emph{vertical} edges of $P$.
Let $C_1\defEQ\bigcup_{P\oftype\PP}\Paren{V_P\cup L_P}$ and 
		$C_2\defEQ\Brace{\iSup{\II}}\cup\Brace{t_2\oftype\Real\filter\exists t_1\oftype\Real\SuchThat\Paren{t_1,t_2}\in C_1}$ be 
    the projection of points in $C_1$ on $t_2$ and $\iSup{\II}$ (if $\iSup{\II}=\infty$ then remove it from $C_2$).
%		
Note that $C_2$ is always a finite set.
Therefore, there is $\epsilon\oftype\pReal$ such that $\II\setminus\infOBall^\epsilon\Paren{C_2}\neq\emptyset$.
Fix any such $\epsilon$ for the rest of this sub-section, and
let $r\oftype\II\setminus\infOBall^\epsilon\Paren{C_2}$ be an arbitrary element.
%
We know for any $P\oftype\PP$ and $c\oftype\Real$, $\Closure{\Sem{P}}\cap\Sem{t_1=c}$ is equal $\Brace{c}\times J$, for some interval $J$.
Define $\Norm{\Closure{\Sem{P}}\cap\Sem{t_1=c}}$ to be $\Norm{J}$.
We prove
	$\exists\delta\oftype\pReal\SuchThat
	 \forall P\oftype\PP,c\oftype\Real\WeHave
	 \Paren{c,r}\in\Closure{\Sem{P}}\Rightarrow
	 \Norm{\Closure{\Sem{P}}\cap\Sem{t_1=c}}\notin\LopRcl{0,8\delta}$.
For the purpose of contradiction, knowing $\PP$ is a finite set, assume
	$\exists P\oftype\PP\SuchThat
	 \forall n\oftype\pNat\WeHave
	 \exists c_n\oftype\Real\SuchThat
	 \Paren{c_n,r}\in\Closure{\Sem{P}}\wedge\Norm{\Closure{\Sem{P}}\cap\Sem{t_1=c_n}}\in\Paren{0,\frac{1}{n}}$.
If $\Sem{P}$ is a point or empty set then its intersection with $\Sem{t_1=c_n}$ is either empty or has width $0$, which is either way a contradiction. 
Otherwise,
if $\Sem{P}$ is a horizontal line, a horizontal half line, or a horizontal line segment, its intersection with $\Sem{t_1=c_n}$ is either empty or has a fixed 
width, which is again a contradiction. Otherwise,
if $\Sem{P}$ is a line, a half line, or a line segment, its intersection with $\Sem{t_1=c_n}$ is either empty or has width $0$, which is another contradiction. 
Otherwise,
$P$ has a non-empty interior and since it has a finite number of vertices, an infinite subsequence of $\Paren{c_n,r}$ converges to a vertex of $P$.
However, this is a contradiction since $\Paren{c_n,r}$ is always $\epsilon$ away from any point in $C_1$.
%
Finally, \wLOG, we assume that $\iSup{\II}-r>4\delta$.

\begin{floatingfigure}[r]{30mm}
\centering
\includegraphics[width=30mm]{./fig-r.pdf}
\vskip-\baselineskip
\caption{}\label{fig:r}
\end{floatingfigure}
\Fig~\ref{fig:r} shows geometrical interpretation of the new constants.
%
For any clause $P\Implies S$ in $\Phi_{\neg p,\neg q,\II}$ and 
for any horizontal line $L$ defined by $t_1=c$ (for an arbitrary constant $c\oftype\Real$),
if $\Paren{c,r}\in\Sem{P}$ then we have two important properties:
\begin{inparaenum}
\item Either $a=b=r$ or at least one of $\Size{r-a}>4\delta$ and $\Size{r-b}>4\delta$ is true. This implies,
\item if $\Sem{P}\cap\Sem{L}\neq\emptyset$ and $S$ contains a constraint of the form $f^{t_2}\OSat\psi$ then either 
			$P\Implies S$ checks the input signal only at $r$, or 
			it						checks an interval of width $>4\delta$ at left, right, or both sides of $r$.
\end{inparaenum}


%%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Constructing Signals $\Sgn_1$ and $\Sgn^\epsilon_2$}\label{sec:signals}
\Fig~\ref{fig:signals} specifies two signals $\Sgn_1$ and $\Sgn^\epsilon_2$.
Every line segment specifies an interval of time.
Empty and filled circles on these line segments, respectively, denote open and closed  endpoints in the corresponding intervals. 
In $\Sgn_1$, the first interval has width equal to $r$, 
				  the next three have width $\delta$, and 
					the last one's width is infinite. 
$\Sgn^\epsilon_2$ is exactly like $\Sgn_1$, except 
	width of the first and second intervals are respectively $r+\epsilon$ and $\delta-\epsilon$, and
	their right/left closeness are swapped.
%In $\Sgn^\epsilon_2$, the first  interval has width equal to $r+\epsilon$, 
%									 the next   one has  width $\delta-\epsilon$, 
%									 the next   two have width $\delta$, and 
%									 the last   one's width is infinite.
Below every line segment is values of atomic propositions in the corresponding interval. 
Finally, it is easy to see that
	$\Sgn_1				 \OSat \neg\Paren{\Until{p}{q}[\II]}$,
	$\Sgn^\epsilon_2\ONSat\neg\Paren{\Until{p}{q}[\II]}$.
Therefore, we must have
	$\Sgn_1				 \NSat \Release{\neg p}{\neg q}[\II]$,
	$\Sgn^\epsilon_2\NNSat\Release{\neg p}{\neg q}[\II]$.
Note that $\Sgn_1$ and $\Sgn^\epsilon_2$ are only different during $\Paren{r,r+\epsilon}$.
%
We specify value of $\epsilon\oftype\Paren{0,\delta}$ precisely in \Sec~\ref{sec:contradiction}.
For now it can be any value that satisfies $r+\epsilon\in\II$
(this is always possible since $C_2$ in \Sec~\ref{sec:consts} contains $\iSup{\II}$). 
%
Note that $f_1$ and $f^\epsilon_2$ change their values only $4$ times throughout $\nnReal$.

\begin{figure}[h]
\centering
  \subfloat[$\Sgn_1$: 
            Since $\Sgn_1\OSat\neg\Paren{\Until{p}{q}[\II]}$, we must have 
                  $\Sgn_1\NSat$\mbox{$\Release{\neg p}{\neg q}[\II]$}.
            \label{fig:signalfs-1}]{%
		\scalebox{0.85}{\input{./fig-signals-1.tex}}}
  \hfill
  \subfloat[$\Sgn^\epsilon_2$: 
            Since $\Sgn^\epsilon_2\ONSat\neg\Paren{\Until{p}{q}[\II]}$, we must have 
                  $\Sgn^\epsilon_2\NNSat$\mbox{$\Release{\neg p}{\neg q}[\II]$}.
            \label{fig:signals-2}]{%
		\scalebox{0.85}{\input{./fig-signals-2.tex}}}
\caption{Signals $\Sgn_1$ and $\Sgn^\epsilon_2$ (interval widths are not proportional).
				 Parameter $\epsilon\oftype\Paren{0,\delta}$ is such that $r+\epsilon\in\II$.}%
\label{fig:signals}
\end{figure}
%\includegraphics[width=0.46\columnwidth]{./fig-signals-1.pdf}}
%\includegraphics[width=0.46\columnwidth]{./fig-signals-2.pdf}}

%%---------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Deriving a Contradiction}\label{sec:contradiction}
Since $\Sgn_1\NSat\Release{\neg p}{\neg q}[\II]$, we know there are $c_1,\ldots,c_n\oftype\Real$ and $j_1,\ldots,j_n\oftype\Nat$ such that for any 
$i\oftype\Brace{1,\ldots,n}$, 
line $L_i\defEQ\Paren{t_1=c_i}$ witnesses $\exists t_1\SuchThat\forall t_2\WeHave\phi_{i,j_i}$.
% 
For any $i\oftype\Brace{1,\ldots,n}$, 
	let $\epsilon_i\oftype\pReal$, 
  clause $P_i\Implies S_i$ from $\phi_{i,j_i}$, and 
			interval $\JJ_i$ be such that
	either $\Brace{c_i}\times\JJ_i = \Sem{P_i}\cap\Sem{L_i}$ and $\Paren{r,r+\epsilon_i}\subseteq\JJ_i$, or 
	$\JJ_i=\emptyset$ in case no such non-empty $\JJ_i$ exists.
Note that Step~\ref{smpl:disjoint} in \Sec~\ref{sec:smpl} guarantees uniqueness of $P_i\Implies S_i$ and $\JJ_i$ whenever $\JJ_i\neq\emptyset$.
%
There must be at least one $i\oftype\Brace{1,\ldots,n}$ such that 
	$\JJ_i\neq\emptyset$,
	$\forall     t_2\oftype\JJ_i\WeHave S_i\Paren{c_i,t_2,\Sgn_1}$, and
	$\forall\epsilon\oftype\pReal\WeHave\neg\forall t_2\oftype\JJ_i\WeHave S_i\Paren{c_i,t_2,\Sgn^\epsilon_2}$.
Otherwise,	$\exists\epsilon\oftype\pReal\SuchThat \Sgn^\epsilon_2\NSat\Release{\neg p}{\neg q}[\II]$ using the exact set of witnesses, which is a contradiction.
Finally, let $\epsilon\defEQ\frac{1}{2}\min\Paren{\Brace{\epsilon_i\filter\JJ_i\neq\emptyset}\cup\Brace{c_i-r\filter c_i>r}}$.

For any $i$ for which $\JJ_i\neq\emptyset$, using \Sec~\ref{sec:consts}, we know at least one of $\iSup{\JJ_i}-r>4\delta$ or $r-\iInf{\JJ_i}>4\delta$ is true.
Recall that $\psi_1$ and $\psi_2$ have no temporal operators.
\begin{myitems}
\item If $\iSup{\JJ_i}-r>4\delta$ then there are three cases for $S_i$, and they are all contradictions since $S_i$ won't reject $\Sgn^\epsilon_2$ 
      (\ie, in all cases $\forall t_2\oftype\JJ_i\WeHave S_i\Paren{c_i,t_2,\Sgn^\epsilon_2}$ is true):
			\begin{myitems}
			\item $S_i$ is of the form $\Sgn^{t_1}\OSat\psi_1$.
            Either $c_i\leq r$ or $c_i>r$ is true and since in both cases $\Sgn_1(c_i)=\Sgn^\epsilon_2(c_i)$, $S_i$ won't reject $\Sgn^\epsilon_2$.
			\item $S_i$ is of the form $\Sgn^{t_2}\OSat\psi_2$.
            Since $L_i$ is a witness and $\forall t_2\oftype\JJ_i\WeHave S_i\Paren{c_i,t_2,\Sgn_1}$ is true,
            definition of $\Sgn_1$ during $\Paren{r,r+4\delta}$ ensures $\psi_2$ is equivalent to $\top$.
			\item $S_i$ is of the form $\Sgn^{t_1}\OSat\psi_1\vee\Sgn^{t_2}\OSat\psi_2$.
            If $\Sgn^{c_i}\OSat\psi_1$ is true then the argument in the first case applies.
            Otherwise, the argument in the second case applies.
			\end{myitems}
\item If $r-\iInf{\JJ_i}>4\delta$ then there are three cases for $S_i$, and they are all contradictions since $S_i$ won't reject $\Sgn^\epsilon_2$:
			\begin{myitems}
			\item $S_i$ is of the form $\Sgn^{t_1}\OSat\psi_1$. 
						The exact same argument as in the case $\iSup{\JJ_i}-r>4\delta$.
			\item $S_i$ is of the form $\Sgn^{t_2}\OSat\psi_2$.
            Since $\Paren{r,r+\epsilon_i}\subseteq\JJ_i$, $\psi_2$ must be true for both $p\wedge\neg q$ and $\neg p\wedge q$.
            Therefore, $S_i$ cannot reject $\Sgn^\epsilon_2$.
%            it must be equivalent to one of
%						$\top$, $p\vee q$, $\neg p\vee\neg q$, or $p\leftrightarrow\neg q$, and none of them rejects $\Sgn^\epsilon_2$.
			\item $S_i$ is of the form $\Sgn^{t_1}\OSat\psi_1\vee\Sgn^{t_2}\OSat\psi_2$.
            If $\Sgn^{c_i}\OSat\psi_1$ is true then the argument in the first case applies.
            Otherwise, the argument in the second case applies.
			\end{myitems}
\end{myitems}

%% Since for any $\epsilon\oftype\pReal$, $f_1$ satisfies $\Release{\neg p}{\neg q}[\II]$ and $f^\epsilon_{13}$ does not, and since these two signals 
%% are only different in $\Paren{r,r+\epsilon}$, we conclude for any $\epsilon\oftype\pReal$ there is a certificate line $L\defEQ\Paren{t_1=c}$ for 
%% $f_1$ that is not a certificate for $f^\epsilon_{13}$. In other words, there is $P\Implies C$ in $\Phi_{\neg p,\neg q,\II}$ such that 
%% $\Brace{c}\times\Paren{r,r+\epsilon'}\subseteq\Sem{L}\cap\Sem{P}$ for some $\epsilon'\oftype\pReal$.
%% %
%% Let $\Sem{L}\cap\Sem{P}$ be $\Brace{c}\times J$ for some interval $J$.
%% %
%% From \Sec~\ref{sec:consts}, we know at least one of $\iSup{J}-r>4\delta$ or $r-\iInf{J}>4\delta$ are true.
%% Next, we consider each case separately:
%% %
%% \begin{myitems}
%% \item If $\iSup{J}-r>4\delta$ then
%% 			since $\Phi_{\neg p,\neg q,\II}$ checks at least $4\delta$ to the right of $r$,
%% 			considering $f_1$ in $\Paren{r,r+4\delta}$, $S$ is equivalent to one of following formulas:
%% 			\begin{inparaenum}
%% 			\item $\Paren{\Sgn^{t_2}\OSat\top}$ which is a contradiction since $P\Implies S$ does not reject $f^\epsilon_{13}$.
%% 			\item $\Paren{\Sgn^{t_1}\OSat\psi_1}\vee\Paren{\Sgn^{t_2}\OSat\top}$ which for the exact same reason is a contradiction.
%% 			\item	$\Paren{\Sgn^{t_1}\OSat\psi_1}$.
%% 			\end{inparaenum}
%% \item If $r-\iInf{J}>4\delta$ then
%% \end{myitems}
%% 
%% 
%% 	$\Paren{\Sgn^{t_1}\OSat\psi_1}\vee\Paren{\Sgn^{t_2}\OSat\top}$
%% 	which is equivalent to the first form.
%% If $c\leq r$ then $P\Implies S$ does not reject $f^\epsilon_{13}$ which is a contradiction.
%% If $c>r$     then $P\Implies S$ does not reject $f_2$ which is a contradiction as well.
%% 
%% Next, assume $r-\iInf{J}>4\delta$ is true.
%% 
%% 
%% Since for any $\epsilon\oftype\pReal$, $\Paren{r,r+\epsilon}$ is open on the left (openness in the right is irrelevant), and 
%% since $\PP$ and number of certificate lines are both finite,
%% there must be $\epsilon\oftype\pReal$, 
%% 							clause $P\Implies S$, and 
%% 							certificate line $L$ at $t_1=c$ such that 
%%   For $C\defEQ\Sem{P}\cap\Sem{L}\cap\Brace{\Paren{c,x}\filter x\oftype\Paren{r,r+\epsilon}}$ we have
%% 	$\Norm{C}>0$ and 
%% 		$\Paren{\forall t_2\oftype C\WeHave S(c,t_1)}$ for $f_1$, and
%% 	  $\neg\Paren{\forall t_2\oftype C\WeHave S(c,t_1)}$ for $f^\epsilon_{13}$.
%% From \Sec~\ref{sec:consts} we know width of $C$ is at least $8\delta$ and distance of $r$ to at least one end points of $C$ is at least $4\delta$.
%% %
%% First assume distance of $r$ to the right end of $C$ is at least $4\delta$.
%% Since $S$ must be satisfied for all values of $f_1$ during $C$, there are two cases:
%% \begin{inparaenum}
%% \item $S$ has no constraint of the form $f^{t_2}\OSat\psi$.
%% 			But this is a contradiction with the fact that for any $\epsilon\oftype\pReal$, $S$ will reject $f^\epsilon_{13}$.
%% \item $S$ has a constraint of the form $f^{t_2}\OSat\psi$.
%% 			But structure of $f_1$ guarantees that $\psi$ is $\top$ which is a contradiction with Step~\ref{smpl:top-free} in \Sec~\ref{sec:smpl}.
%% \end{inparaenum}
%% Therefore, distance of $r$ to the left point of $C$ must be at least $4\delta$ (we only use the fact that this distance is positive). 
%% There are $16$ possible cases for $\psi$ and we consider them all next:
%% \begin{myitems}
%% \item $\top$: this is a contradiction since in this case $\psi$ is satisfied by $f^\epsilon_{13}$. 
%% \item $\bot$, $p$, $q$, $p\wedge q$, $p\wedge\neg q$, $\neg p\wedge q$, $\neg p\wedge\neg q$, $p\vee\neg q$, $\neg p\vee q$, $p\leftrightarrow\neg q$: this is a contradiction since in this case $\psi$ is not satisfied by $f_1$.
%% \item $p\vee q$, $\neg p\vee\neg q$, $p\leftrightarrow q$: this is a contradiction since $\psi$ does not reject $f_2$.
%% \end{myitems}
%% 
%% \subsection{When $\Psi$ is Nested}\label{sec:nested}
%% Since semantics of $\UntilOp$, as defined in \Def~\ref{def:mtl-sem}, can be easily expressed using the syntax in \Thm~\ref{thm:2vars}, we know every interval in $\Psi$ has either size $0$ or larger than $8\delta$.


==> part-3vars.tex <==
\section{Three Variables Are Enough}\label{sec:3vars}
In \Sec~\ref{sec:2vars} we proved using two variables one cannot make $\UntilOp$ and $\ReleaseOp$ dual of each other.
In this section, we redefine semantics of $\ReleaseOp$ using three variables and prove that it guarantees duality of all operators.
%
Denseness of time as well as openness and closeness of intervals in both signals and \MTL\ formulas have proven themselves to be a serious
subtleties for establishing facts about \MTL. In order to increase confidence, we have already proved many of our positive results in 
Prototype Verification System (\PVS)~\cite{92-PVS}.
%
We explicitly mark all lemmas and theorems that fall in this category and for the sake of space remove proofs from this paper~\footnote{%
Each of these marks is in the form of $\langle\textsf{lemma-name}\rangle@\langle\textsf{theory-name}\rangle$.
Theory name \textsf{thry} can be found in a file named \textsf{thry.pvs}.}.
All formal proofs can be found at \url{https://uofi.box.com/v/PVSProofsOfMITL}.


\begin{definition}[New Semantics for \MTL]\label{def:mtl-newsem}
Let $\Sgn\oftype\nnReal\goesto\pset{\AP}$ be an arbitrary signal and $r\oftype\nnReal$ be an arbitrary point in time.
For a \MTL\ formula $\varphi$, we define satisfaction relation $\Sgn\NSat\varphi$ using the following inductive rules: 
\[
\newcommand{\DEF}{\mbox{\ \iFF\ }}
\begin{array}{@{}lll@{}}
\Sgn\NSat\top                                 &\DEF&\top\\
\Sgn\NSat\bot                                 &\DEF&\bot\\
\Sgn\NSat p                                   &\DEF&p\in\Sgn(0)\\
\Sgn\NSat\neg\varphi                          &\DEF&\neg\Paren*{\Sgn\NSat\varphi}\\
\Sgn\NSat\varphi_1\vee  \varphi_2             &\DEF&\Paren*{\Sgn\NSat\varphi_1}\vee  \Paren*{\Sgn\NSat\varphi_2}\\
\Sgn\NSat\varphi_1\wedge\varphi_2             &\DEF&\Paren*{\Sgn\NSat\varphi_1}\wedge\Paren*{\Sgn\NSat\varphi_2}\\
\Sgn\NSat\Until{\varphi_1}{\varphi_2}[\II]    &\DEF&\exists t_1\oftype\II\SuchThat\Paren*{\Sgn^{t_1}\NSat\varphi_2}\wedge
                                                    \forall t_2\oftype\Paren{0,t_1}\WeHave\Sgn^{t_2}\NSat\varphi_1\\
\Sgn\NSat\Release{\varphi_1}{\varphi_2}[\II]  &\DEF&\forall t_1\oftype\II\WeHave\Sgn^{t_1}\NSat\varphi_2\ \ \ \vee\\
                                              &    &\exists t_1\oftype\pReal\SuchThat\Paren*{\Sgn^{t_1}\NSat\varphi_1}\wedge
                                                    \forall t_2\oftype\Braket{0,t_1}\cap\II\WeHave\Sgn^{t_2}\NSat\varphi_2\ \ \ \vee\\
                                              &    &\exists t_1\oftype\CloseL{\II},t_2\oftype\II\cap\Paren{t_1,\infty}\SuchThat
                                                    \forall t_3\oftype\II\WeHave\Paren{t_3\leq t_1\Implies\Sgn^{t_3}\NSat\varphi_2}\\
                                              &    &\hfill\wedge\Paren{t_1 < t_3\leq t_2\Implies\Sgn^{t_3}\NSat\varphi_1}
\end{array}
\]
$\Sgn\NNSat\varphi$ is defined to be $\neg\Paren*{\Sgn\NSat\varphi}$.
\end{definition}

As expected, \Def~\ref{def:mtl-newsem} only changes semantics of $\ReleaseOp$ operator.
Decision procedures only considers signals that are finite variable with respect to every \MTL\ sub-formula.
However, most of the times, a user of those procedures can only guarantees finite variability of atomic propositions.
\Lem~\ref{lem:fvar} states these two remain equivalent.
 

\PVSaddress{%
  \PVSLabel*{mtl}{atom\_finitevar\_eqv\_fml\_finitevar\_left} and
\PVSLabel{mtl}{atom\_finitevar\_eqv\_fml\_finitevar\_right}}
\newcommand{\RESfvar}{%
Using the semantics in \Def~\ref{def:mtl-newsem}, for any signal $\Sgn$, the following conditions hold:
\[
\begin{split}
  \Paren*{\forall p\oftype\AP\WeHave\fvarL[\Sgn,p]}\Leftrightarrow\Paren*{\forall \varphi\oftype\MTL\WeHave\fvarL[\Sgn,\varphi]}\\
  \Paren*{\forall p\oftype\AP\WeHave\fvarR[\Sgn,p]}\Leftrightarrow\Paren*{\forall \varphi\oftype\MTL\WeHave\fvarR[\Sgn,\varphi]}
\end{split}
\]}
\begin{pvslemma}[Finite Variability]\label{lem:fvar}
\RESfvar
\end{pvslemma}

%\PVSaddress{\PVSLabel{mtl}{sat\_implies\_nnfsat}}
%\newcommand{\RESDualityOne}{%
%  For any signal $\Sgn$ that is finitely variable from right and \MTL\ formula $\varphi$ we have $\Sgn\NSat\varphi$ implies $\Sgn\NSat\nnf[\varphi]$.}
%\begin{pvslemma}[Duality-1]\label{lem:duality-1}
%\RESDualityOne
%\end{pvslemma}


%\PVSaddress{\PVSLabel{mtl}{nnfsat\_implies\_sat}}
%\newcommand{\RESDualityTwo}{%
%  For any signal $\Sgn$ and \MTL\ formula $\varphi$ we have $\Sgn\NSat\nnf[\varphi]$ implies $\Sgn\NSat\varphi$.}
%\begin{pvslemma}[Duality-2]\label{lem:duality-2}
%\RESDualityTwo
%\end{pvslemma}

\PVSaddress{\PVSLabel{mtl}{sat\_eqv\_nnfsat}}
\newcommand{\RESnnfEqvSat}{%
  If a signal $\Sgn$ is finitely variable from right then for any \MTL\ formula $\varphi$, $\Sgn\NSat\varphi$ \iFF\ $\Sgn\NSat\nnf[\varphi]$.}
\begin{pvstheorem}[Duality]\label{thm:duality}
  \RESnnfEqvSat
\end{pvstheorem}

We next define a new temporal operator that will be useful in more than one place.
For any \MTL\ formula $\varphi$, let $\ltlN\varphi$ be defined as $\Release{\varphi}{\varphi}[\Paren{0,\infty}]$.
Intuitively, $\Sgn\NSat\ltlN\varphi$ \iFF\ $\varphi$ becomes true and stays true for some positive amount of time.
\Prop~\ref{prop:next} formalizes this property.
Note that instead if $\infty$ in definition of $\ltlN\varphi$, one can use any other positive number and obtain an equivalent 
formula~\footnote{\label{ft:next}\PVSLabel*{mtl}{next\_def\_1}, \PVSLabel{mtl}{next\_def\_3}}.
Finally, assume $\ltlN$ has higher precedence over $\UntilOp$ and $\ReleaseOp$ operators and lower precedence over $\vee$ and $\wedge$ operators. 

\PVSaddress*{ft:next}
\newcommand{\RESnext}{%
  Let $\Sat$ be the satisfaction relation defined in \Def~\ref{def:mtl-sem} or \Def~\ref{def:mtl-newsem}.
  For any signal $\Sgn$ we have 
  $\Sgn\Sat\ltlN\varphi$ \iFF\ 
  $\exists\epsilon\oftype\pReal\SuchThat\forall t\oftype\Paren{0,\epsilon}\WeHave\Sgn^t\Sat\varphi$.}
\begin{pvsproposition}[Operator \ltlN]\label{prop:next}
\RESnext
\end{pvsproposition}


We end this section by \Ex~\ref{ex:fvar-nnf} that shows, as far as \Def~\ref{def:mtl-newsem} is concerned, we cannot completely get rid of finite 
variability condition. We leave existence of a $\exists\forall$ semantics for $\ReleaseOp$ operator that guarantees equivalency of a formula with its \NNF, 
without any finite variability condition, as an open question.

\begin{example}\label{ex:fvar-nnf} 
Let $\varphi$ be the following formula.
Then $\varphi$ is satisfiable by a signal that is finitely variable from left, but it is not satisfiable by any signal that is finitely variable from
right.
\[\Paren*{\ltlN q}\wedge\neg\Paren*{\Until{p}{q}[\Paren{0,1}]}\wedge\neg\Paren*{\Until{\neg p}{q}[\Paren{0,1}]}\]
Putting $\varphi$ into its \NNF\ we obtain the following formula which is not satisfiable 
(using either \Def~\ref{def:mtl-sem} or \Def~\ref{def:mtl-newsem}).
\[\Paren*{\ltlN q}\wedge\Paren*{\Release{\neg p}{\neg q}[\Paren{0,1}]}\wedge\Paren*{\Release{p}{\neg q}[\Paren{0,1}]}\]
\end{example}


==> part-mitlwi-old.tex <==
%\MakeGrayColorDarker%must be at the end of Sec~{sec:reduction}
\section{\MITL\ with Wide Intervals (\MITLwi)}\label{sec:MITLwi}
Let \MITLwi\ be a subclass of \MITL\ formulas in which for every interval $\II$ used in a formulas $\varphi$, if $0<\iInf{\II}<\iSup{\II}<\infty$ then 
$\frac{\iSup{I}}{\iSup{I}-\iInf{I}}\leq n$, where $n$ is the size of $\varphi$ with binary constants.
Also, as opposed to natural numbers in~\cite{96-MITL}, in this section we allow constants to be rational numbers.
Clearly, every \MITLzi\ formula is a \MITLwi\ formula, but there are lots of \MITLwi\ formulas that are not in \MITLzi.
%
The main result of this section is in \aref{cor:MITLwi} which is an immediate consequence of \aref{thm:MITLwi}.
It would be helpful to first see why \MITL\ is exponentially more complex than \MITLzi, and that is what we do in \aref{sec:MITLvsMITLzi}.
In \aref{sec:witness} we prove \aref{thm:MITLwi} by showing \MITLwi\ does not suffer from complexity of \MITL.

\begin{theorem}\label{thm:MITLwi}
For any \MITLwi\ formula $\varphi$ of size $n$, there is a \TAls\ $\Sem{\varphi}$ such that a signal $\Sgn$ is in the language of $\Sem{\varphi}$ \iFF\ 
$\fvar[\varphi]$ and $\Sgn\NSat\varphi$.
Furthermore, $\Sem{\varphi}$ can be constructed in polynomial space and has the following properties:
\begin{myenums}
\item it has at most $2^{\BigO[n^2]}$ many locations and edges,
\item it has at most $\BigO[n]$ many clocks,
\item it has at most $\BigO[n]$ many distinct integer constants, each bounded by $2^{\BigO[n]}$.
\end{myenums}
\end{theorem}

\begin{corollary}\label{cor:MITLwi}
Model checking and satisfiability problems for \MITLwi\ is \PSPACEcomp.
\begin{proof}
Being in \PSPACE\ is an immediate consequence of \aref{thm:MITLwi}, and 
being in \PSPACEhard\ is because the same problems for \MITLzi\ are \PSPACEhard.
\end{proof}
\end{corollary}

%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{\MITL\ vs. \MITLzi}\label{sec:MITLvsMITLzi}
In order to transform a \MITL\ formula into a \TAls, authors in~\cite{96-MITL} first apply a series of syntactic transformations such that the result formula
\begin{inparaenum}
\item is in negated normal form,
\item has at most linearly more distinct subformulas,
\item has the same maximum constant as the original formula, and most importantly, 
\item is in normal form which is specified in \aref{def:nf}.
\end{inparaenum}
After introducing these transformations and showing they can be easily done in polynomial time, they assume that the input formula is already given in the 
normal form.
They also show that the input formula and hence its normal form is in \MITLzi\ \iFF\ it has no subformula of \aref{typ:nfUntil} and \aref{typ:nfRelease}, as
specified in \aref{def:nf}.

\begin{definition}[Normal Form~\mbox{\cite[\Def~4.1]{96-MITL}}]\label{def:nf}
\MITL\ formula $\varphi$ is in {\em normal form} \iFF\ it is built from propositions and negated propositions using conjunction,
disjunction, and temporal subformulas of the following six types:
\vfil\penalty999\vfilneg%For some reason, page will break here if you comment this line
\begin{multicols}{2}
\begin{myenums}
\item\label{typ:nfFinally} $\ltlF_\II\varphi'$ with $\IsLOpen{\II}$, $\iInf{\II}=0$, and $\iSup{\II}\in\Real$,
\item\label{typ:nfAlways}  $\ltlG_\II\varphi'$ with $\IsLOpen{\II}$, $\iInf{\II}=0$, and $\iSup{\II}\in\Real$,
\item\label{typ:nfAllTime} $\ltlG\varphi'$.
\item\label{typ:nfUntil}   $\Until  {\varphi_1}{\varphi_2}[\II]$ with $\iInf{\II}>0$, and $\iSup{\II}\in\Real$,
\item\label{typ:nfRelease} $\Release{\varphi_1}{\varphi_2}[\II]$ with $\iInf{\II}>0$, and $\iSup{\II}\in\Real$,
\item\label{typ:nfUntil2}  $\Until{\varphi_1}{\varphi_2}$,
\end{myenums}
\end{multicols}
\end{definition}

To see the difficulty of transforming \aref{typ:nfUntil} and \aref{typ:nfRelease} formulas into \TAlp, consider 
$\ltlG_{\Opened{3,4}}\Paren{p\rightarrow\ltlF_{\Opened{1,2}}q}$.
Intuitively, the formula says, during the $4$\textsuperscript{th} unit of time, every $p$ should be followed by a $q$ within $1$ to $2$ units of time.
A na\"ive approach, starts and dedicates a clock after seeing every $p$ during $4$\textsuperscript{th} unit of time, and use that clock to make sure there 
will be at least one $q$, $1$ to $2$ units of time after the corresponding $p$ was seen.
However, this approach does not work, since there is no bound on number of $p$ that one can expect to see during any period of time, which makes number of 
required clocks infinite.

Instead, authors in~\cite{96-MITL} divide $\nnReal$ into $\LclRop{0,1},\LclRop{1,2},\ldots$ intervals and prove two important
facts about them:
\begin{inparaenum}
\item For any interval $\LclRop{n,n+1}$ and any \aref{typ:nfUntil} $\UntilOp$ or \aref{typ:nfRelease} $\ReleaseOp$ formula $\varphi$, 
			the subset of times in $\LclRop{n,n+1}$ for which $\varphi$ is true is exactly union of two possibly empty intervals.
			Using this property, for each interval $\LclRop{n,n+1}$, we first guess those two intervals and then use at most $4$ clocks to verify our guess.
\item We can start reusing a clock at most $\iSup{\II}$ units of time after we started using it.
			Therefore, total number of clocks required for checking each \aref{typ:nfUntil} and \aref{typ:nfRelease} formula is bounded by $4\iSup{\II}$.
\end{inparaenum}
Since $\iSup{\II}$ could be exponentially big, the result \TAls\ could have exponentially many clocks, which makes its emptiness check \EXPSPACEcomp~\footnote{%
	According to~\cite{96-MITL}, one should also keep track of the subset of clocks that are free (\ie\ can be reused).
	A na\"ive\ approach (as taken in~\cite{96-MITL}), just encodes this subset in discrete modes of the result \TAls\ which makes the	number of locations doubly 
	exponential.
	However, it is possible to reuse clocks in a queue like fashion and instead of encoding a subset of free clocks in discrete	modes, just encode index of the 
	next free clock.
	This approach exponentially decreases number of required discrete modes.
	Either way, \EXPSPACE\ is still enough to check emptiness of the result \TAls.}. 

%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Witness Points and Intervals}\label{sec:witness}
In this section, let {\em step size} of an interval, denoted by $\Step[\II]$, be defined according to \aref{eq:step}.
We show that \aref{typ:nfUntil} and \aref{typ:nfRelease} formulas are actually a lot less variable.
Meaning, if $\II$ is a bounded non-empty interval with $\iInf{\II}>0$ then instead of considering intervals 
$\LclRop{0,1},\LclRop{1,2},\ldots$ one can consider intervals $\LclRop{0,c},\LclRop{c,2c},\ldots$, where $c\defEQ\Step[\II]$.
There will be two important consequences:
\begin{myenums}
\item If a formula is in \MITLwi, then number of required clocks will be at most linear in the size of formula.
			For example, verifying $\ltlG_{\Closed{n,2n}}\varphi$ requires constant number of clocks, as opposed to exponentially many clocks in~\cite{96-MITL}.
\item Consider satisfiability of $\varphi\defEQ\ltlG_{\Closed{1,2}}\ltlF_{\Closed{0.01,0.02}}\varphi'$ formula.
	    According to~\cite{96-MITL}, we need to first write $\varphi$ as an equivalent formula 
			$\varphi\defEQ\ltlG_{\Closed{100,200}}\ltlF_{\Closed{1,2}}\varphi'$, since dividing $\nnReal$ into 
			$\LclRop{0,1},\LclRop{1,2},\ldots$ assumes all constants in the input formula are natural numbers.
			Therefore, \TAls\ will have hundreds of clocks.
			However, we show there is no need for interval end points to be natural numbers, and \TAls\ for $\varphi$ requires at most
			$8$ clocks for each of $\ltlG_{\Closed{1,2}}$ and $\ltlF_{\Closed{0.01,0.02}}$ formulas.
			Note that model checking the result \TAls, requires replacing all rational numbers by natural numbers.
			But the point is that, as far as emptiness problem for \TAlp\ is concerned, increasing clocks is exponentially worse than 
			increasing constants~\cite[\Lem~4.5]{94-TA}.
\end{myenums}

\begin{equation}\label{eq:step}
\Step[\II]\defEQ\left\{
\begin{array}{@{}l@{\ \ \ }l@{}}
	\iSup{\II}-\iInf{\II} & \mbox{if }\iSup{\II}-\iInf{\II}<\iInf{\II}	\\
	\iInf{\II}            & \mbox{otherwise}
\end{array}
\right.
\end{equation}

%\setcounter{secnumdepth}{3}
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Witness Points for \UntilOp\ Operators.}\label{sec:Uwitness}


%In this section we present few results on satisfiability of $\UntilOp$ and $\ReleaseOp$ operators, and
%in \aref{sec:ta} we introduce a new method for transforming \MITL\ formulas into equivalent timed automata.
%The transformation method devised in \aref{sec:reduction} (based on the one in~\cite{96-MITL}), has few problems and the new procedure solve 
%them all.
%\begin{inparaenum}
%\item It constructs an exponentially large formula which although does not change the complexity, multiplies number of steps by an exponential factor.
%\item For any $n\oftype\Brace{2,3,\ldots}$ checking satisfiability of $\Until{p}{q}[\Paren{1,n}]$	requires about $4n$ clocks. Which is the sole reason 
%			for	\EXPSPACE\ complexity of \MITL\ satisfiability problem.
%			The new decision procedure requires about $\frac{2\iSup{\II}}{\iSup{\II}-\iInf{\II}}$ clocks which is exponentially smaller than $4n$ in 
%			lots of situations. 
%\item It requires all constants to be integers.
%			In order to convert a rational interval into an integer interval, it multiplies all constants by the least common multiple of all denominators.
%			For example, $\Paren{\frac{1}{17},\frac{12}{13}}$ will be transformed to $\Paren{13,204}$ which requires about $804$ clocks.
%			The new procedure, support rational numbers as well.
%			In fact it support all real numbers and construct an equivalent timed automaton.
%			However it is well known that even safety problem for timed automata with irrational numbers is undecidable~\cite{00-irTA}.
%\end{inparaenum}

%For the rest of this section, fix 
%	$\Sgn$ as an arbitrary signal,
%	$\varphi_1$ and $\varphi_2$ as two arbitrary \MTL\ formulas, and
%	\II\ as a non-empty interval such that $\iInf{\II},\iSup{\II}\in\pReal$.
For the rest of this section, let $\Sgn$ be an arbitrary signal.
%
\aref{def:until-witness}   defines three sets of pairs  in $\nnReal^2$, each called an \emph{until witness set}.
\aref{def:until-proofset}  defines three sets of points in time, called \emph{until proof set}.
\aref{prop:until-proofset} states  that for any time $r$ in an until proof set, we have $\Sgn^r\NSat\Until{\varphi_1}{\varphi_2}[\II]$.
\aref{thm:until-fv}        proves  the finite variability of $\UntilOp$ formulas, and
\aref{thm:until-witness-point} shows how to use previous theorem to check $\UntilOp$ formulas.
%
Note that $\varphi_1$ and $\varphi_2$ used in the rest of this section, could be any \MTL\ formulas. Also,
in both \aref{prop:until-proofset} and \aref{thm:until-fv}, there is no need for signal $\Sgn$ to be finitely variable.

\begin{definition}[Witness Sets for \UntilOp]\label{def:until-witness}
For every \MTL\ formulas $\varphi_1$ and $\varphi_2$, and 
					$i\oftype\Brace{1,2,3}$, 
we define $\Uwitness^i\Paren{\varphi_1,\varphi_2}$ to be a subset of $\nnReal^2$ defined by the following predicates over $\Paren{r,w}$:
\begin{myenums}
\item $r\leq w \wedge \Paren*{\forall t\oftype\Paren{r,w}\WeHave\Sgn^t\NSat\varphi_1}\wedge\Sgn^w\NSat\varphi_2$
\item $\begin{array}[t]{@{}l@{}l@{}}
				r<w \wedge 
				\exists\epsilon\oftype\pReal\SuchThat
            \Paren*{\forall t\oftype\Paren{r,w}\WeHave\Sgn^t\NSat\varphi_1} & \wedge
%            \Paren*{\forall t\oftype\Paren{\makebox[0pt][l]{$r,w$}\phantom{r,w+\epsilon}}\WeHave\Sgn^t\NSat\varphi_1} & \wedge
						\Paren*{\forall t\oftype\Paren{                           w\Minos\epsilon ,w}\WeHave\Sgn^t\NSat\varphi_2}
			\end{array}$
\item $\begin{array}[t]{@{}l@{}l@{}}
				r<w \wedge 
				\exists\epsilon\oftype\pReal\SuchThat
            \Paren*{\forall t\oftype\Paren{\makebox[0pt][l]{$r,w+\epsilon$}\phantom{r,w+\epsilon}}\WeHave\Sgn^t\NSat\varphi_1} & \wedge
						\Paren*{\forall t\oftype\Paren{w							              						 ,w+\epsilon }\WeHave\Sgn^t\NSat\varphi_2}
			\end{array}$
\end{myenums}
\end{definition}
 

\begin{definition}[Proof Sets for \UntilOp]\label{def:until-proofset}
For every \MTL\ formulas $\varphi_1$ and $\varphi_2$,
					times $r,w\oftype\nnReal$,
					interval $\II\oftype\nnII$, and
					$i\oftype\Brace{1,2,3}$, 
we define $\Uproofset^i\Paren{\varphi_1,\varphi_2,r,w,\II}$ to be a subset of $\nnReal$ defined by the following predicates 
over $t$:
\begin{myenums}
\item $\Uwitness^1\Paren{r,w}\wedge r\leq t\wedge w-t\in\II$
\item $\Uwitness^2\Paren{r,w}\wedge r\leq t\wedge w-t\in\OpenLCloseR{\II}$
\item $\Uwitness^3\Paren{r,w}\wedge r\leq t\wedge w-t\in\OpenRCloseL{\II}$
\end{myenums}
\end{definition}

\newcommand{\RESUProofSet}{%
For any \MTL\ formulas $\varphi_1$ and $\varphi_2$,
				times $r,w\oftype\nnReal$,
				interval $\II\oftype\nnII$, 
				$i\oftype\Brace{1,2,3}$, and
				$t\oftype\Uproofset^i\Paren{\varphi_1,\varphi_2,r,w,\II}$
we have $\Sgn^t\NSat\Until{\varphi_1}{\varphi_2}[\II]$.}
\PVSaddress{\PVSLabel{mtl\_witness}{def\_until\_witness\_\{1,2,3\}\_proofset}}
\begin{pvsproposition}[Proof Sets for \UntilOp]\label{prop:until-proofset}
\RESUProofSet
\end{pvsproposition}


\newcommand{\RESUfvar}{%
For any \MTL\ formulas $\varphi_1$ and $\varphi_2$, and
				interval $\II\oftype\Brace{\II\oftype\allII\filter\iInf{\II},\iSup{\II}\in\pReal}$,
there are two intervals $T_1\oftype\nnII$ and $T_2\oftype\nnII$ with the following properties:
\begin{myitems}
\item $\forall t_1\oftype T_1,t_2\oftype T_2\WeHave t_1<t_2$, and
\item $\forall t\oftype\nnReal\WeHave \Paren*{t<\Step[\II]\wedge\Sgn^t\NSat\Until{\varphi_1}{\varphi_2}[\II]}\Leftrightarrow\Paren{t\in T_1\cup T_2}$
\end{myitems}}
\PVSaddress{\PVSLabel{mtl\_witness}{until\_witness\_interval\_2}}
\begin{pvstheorem}[Finite Variability of \UntilOp]\label{thm:until-fv}
\RESUfvar
\end{pvstheorem}
%The first property states that $T_1$ and $T_2$ are disjoint and $T_1$ happens before $T_2$.
%The second property states that $T_1\cup T_2$ are exactly the set of points that are $<\Step[\II]$ and
%$\Until{\varphi_1}{\varphi_2}[\II]$ are true for them.

\aref{def:until-witness}, defines what should be guessed.
In \aref{thm:until-witness-point}, 
	1\textsuperscript{th} property bounds possible values of $w_i$, and hence bounds possible values that should be guessed by \TAls.
	2\textsuperscript{nd} property specifies what $w_i$ should satisfies (\ie\ what \TAls\ should verify about the guess), and
	3\textsuperscript{rd} property states that $w_i$ is enough for proving $\Until{\varphi_1}{\varphi_2}[\II]$ is satisfied by $\Sgn$ at all times in
	$T_i$.
Note that every result in this section uses \aref{def:mtl-newsem}.
However, everything directly applies to \aref{def:mtl-sem} as well, since we had no assumption on $\varphi_1$ and $\varphi_2$.
In particular, they can be abstracted by two atomic propositions $p$ and $q$.

\newcommand{\RESUwitness}{%
In \aref{thm:until-fv}, if $\fvar[\Sgn]$ then $T_1$ and $T_2$ have the following properties:
\begin{myitems}
\item If $T_1\neq\emptyset$ then there are $w_1\oftype\pReal$ and $i\oftype\Brace{1,2}$ such that:
			\begin{myenums}
			\item if $i=1$ then $w_1-\iInf{T_1}\in\II$, otherwise, $w_1-\iInf{T_1}\in\CloseR{\II}$
			\item $\Paren{\iInf{T_1},w_1}\in\Uwitness^i\Paren{\varphi_1,\varphi_2}$
			\item $T_1\subseteq\Uproofset^i\Paren{\varphi_1,\varphi_2,\iInf{T_1},w_1}$
			\end{myenums}
\item If $T_2\neq\emptyset$ then there are $w_2\oftype\pReal$ and $i\oftype\Brace{1,3}$ such that:
			\begin{myenums}
			\item $w_2-\iInf{T_2}\in\CloseR{\II}$
			\item $\Paren{\iInf{T_2},w_2}\in\Uwitness^i\Paren{\varphi_1,\varphi_2}$
			\item $T_2\subseteq\Uproofset^i\Paren{\varphi_1,\varphi_2,\iInf{T_2},w_2}$
			\end{myenums}
\end{myitems}}
\PVSaddress{\PVSLabel{mtl\_witness}{until\_witness\_interval\_3}}
\begin{pvstheorem}[Witness Point for \UntilOp]\label{thm:until-witness-point}
\RESUwitness
\end{pvstheorem}


%--------------------------------------------------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsubsection{Witness Intervals for \ReleaseOp\ Operators.}\label{sec:Rwitness}
Everything we did for \UntilOp\ operator in the previous section, we repeat here for \ReleaseOp\ operator. 
%
\aref{def:release-witness}   defines four sets of intervals, each called a \emph{release witness set}.
\aref{def:release-proofset}  defines four sets of points in in time, called \emph{release proof set}.
\aref{prop:release-proofset} states  that for any time $r$ in an release proof set, we have $\Sgn^r\NSat\Release{\varphi_1}{\varphi_2}[\II]$.
\aref{thm:release-fv}        proves  the finite variability of $\ReleaseOp$ formulas, and
\aref{thm:release-witness-interval} shows how to use previous theorem to check $\ReleaseOp$ formulas.
%
Note that $\varphi_1$ and $\varphi_2$ used in the rest of this section, could be any \MTL\ formulas. Also,
in both \aref{prop:release-proofset} and \aref{thm:release-fv}, there is no need for signal $\Sgn$ to be finitely variable.


	
\begin{definition}[Witness Interval for \ReleaseOp]\label{def:release-witness}
For every \MTL\ formulas $\varphi_1$ and $\varphi_2$, and 
					$i\oftype\Brace{1,\ldots,4}$, 
we define $\Rwitness^i\Paren{\varphi_1,\varphi_2}$ to be a subset of $\IIc$ defined by the following predicates over \II:
\[
\setcounter{enumi}{0}
\newcommand{\Bullet}{\stepcounter{enumi}\mbox{\labelenumi}}
\begin{array}{@{}l@{\hspace{\labelsep}}l@{}l@{}l@{}}
\Bullet&\multicolumn{3}{@{}l@{}}{\forall t\oftype\II\WeHave\Sgn^t\NSat\varphi_2}\\
\Bullet&				\II &\neq\emptyset\wedge\IsLClosed{\II}	&\wedge\forall t\oftype\II\WeHave\Sgn^t\NSat\varphi_1\\
\Bullet&				\II &\neq\emptyset\wedge\IsRClosed{\II}	&\wedge\forall t\oftype\II\WeHave\Sgn^t\NSat\varphi_2\wedge\Sgn^{\iSup{\II}}\NSat\varphi_1\\
\Bullet&\CloseL{\II}&\neq\emptyset\wedge\IsRClosed{\II}	&
			\wedge\forall t\oftype\II\WeHave\Sgn^t\NSat\varphi_2\wedge\exists\epsilon\oftype\pReal\SuchThat
			 \forall t\oftype\Paren{\iSup{\II},\iSup{\II}+\epsilon}\WeHave
			 \Sgn^t\NSat\varphi_1
\end{array}	
\]
\end{definition}


\begin{definition}[Proof Sets for \ReleaseOp]\label{def:release-proofset}
For every \MTL\ formulas $\varphi_1$ and $\varphi_2$,
          intervals $\II,\JJ\oftype\nnII$, and
          $i\oftype\Brace{1,2,3,4}$, 
we define $\Uproofset^i\Paren{\varphi_1,\varphi_2,\II,\JJ}$ to be a subset of $\nnReal$ defined by the following predicates over $t\oftype\nnReal$:
\[
\setcounter{enumi}{0}
\newcommand{\Bullet}{\stepcounter{enumi}\mbox{\labelenumi}}
\begin{array}{@{}l@{\hspace{\labelsep}}l@{}l@{}l@{}}
\Bullet&	\II\in\Rwitness^1\Paren{\varphi_1,\varphi_2}\wedge&	t+\JJ\subseteq\II\\
\Bullet&	\II\in\Rwitness^2\Paren{\varphi_1,\varphi_2}\wedge& t+\JJ\subseteq\Paren{\iInf{\II},\infty} &\wedge	t<   \iSup{\II}\wedge\iInf{\JJ}>0\\
\Bullet&	\II\in\Rwitness^3\Paren{\varphi_1,\varphi_2}\wedge&	t+\JJ\subseteq\II+\nnReal								&\wedge	t<   \iSup{\II}\\
\Bullet&	\II\in\Rwitness^4\Paren{\varphi_1,\varphi_2}\wedge& t+\JJ\subseteq\II+\nnReal								&\wedge	t\leq\iSup{\II}
\end{array}
\]
\end{definition}


\PVSaddress{\PVSLabel{mtl\_witness}{def\_release\_witness\_\{1,2,3,4\}\_proofset}}
\begin{pvsproposition}[Proof Sets for \ReleaseOp]\label{prop:release-proofset}
For any \MTL\ formulas $\varphi_1$ and $\varphi_2$,
        intervals $\II,\JJ\oftype\nnII$,
        $i\oftype\Brace{1,2,3,4}$, and
				$t\oftype\Rproofset^i\Paren{\varphi_1,\varphi_2,\II,\JJ}$
we have $\Sgn^t\NSat\Release{\varphi_1}{\varphi_2}[\JJ]$.				
\end{pvsproposition}

 
\PVSaddress{\label{ft:release}\PVSLabel{mtl\_witness}{release\_witness\_interval\_1}}
\begin{pvstheorem}[Finite Variability of \ReleaseOp]\label{thm:release-fv}
For any \MTL\ formulas $\varphi_1$ and $\varphi_2$, and
        non-empty positive bounded interval \II, 
there are four intervals $T_1,\ldots,T_4$ with the following properties:
%\setitemize{leftmargin=*}
\setlength{\labelsep}{0.pt}
\begin{myitems}
\item $\forall i,j\oftype\Brace{1,\ldots,4}, t_i\oftype T_i,t_j\oftype T_j\WeHave i<j\Rightarrow t_i<t_j$, and
\item $\forall t\oftype\nnReal\WeHave \Paren*{t<\Step[\II]\wedge\Sgn^t\NSat\Release{\varphi_1}{\varphi_2}[\II]}\Leftrightarrow
	\Paren{t\in\bigcup_{i\oftype{1,\ldots,4}} T_i}$
\end{myitems}
\end{pvstheorem}


\PVSaddress*{ft:release}
\begin{pvstheorem}[Witness Interval for \ReleaseOp]\label{thm:release-witness-interval}
In \aref{thm:release-fv}, if $\fvar[\Sgn]$ then $T_1,\ldots,T_4$ have the following properties:
\begin{multicols}{2}
\begin{myitems}
\item If $T_1\neq\emptyset$ then $\exists\II\oftype\IIc$ such that:
			\begin{myenums}
			\item $\II\subseteq\Paren{0,\Step[\JJ]}$
			\item $\Rwitness^2\Paren{\varphi_1,\varphi_2,\II}$
			\item $T_1\subseteq\Rproofset^2\Paren{\varphi_1,\varphi_2,\II,\JJ}$
			\end{myenums}
\item If $T_2\neq\emptyset$ then $\exists\II\oftype\IIc$ such that:
			\begin{myenums}
			\item $\II\subseteq\LclRop{\Step[\JJ],\Step[\JJ]+\iSup{\JJ}}$
			\item $\Rwitness^1\Paren{\varphi_1,\varphi_2,\II}$
			\item $T_2\subseteq\Rproofset^1\Paren{\varphi_1,\varphi_2,\II,\JJ}$\\
			\end{myenums}
\item If $T_3\neq\emptyset$ then $\exists\II\oftype\IIc$ such that:
			\begin{myenums}
			\item $\II\subseteq\LclRop{\Step[\JJ],\Step[\JJ]+\iSup{\JJ}}$
			\item $\Rwitness^4\Paren{\varphi_1,\varphi_2,\II}$
			\item $T_3\subseteq\Rproofset^4\Paren{\varphi_1,\varphi_2,\II,\JJ}$
			\end{myenums}
\item If $T_4\neq\emptyset$ then $\exists\II\oftype\IIc,i\oftype\Brace{2,3,4}$ such that:
			\begin{myenums}
			\item $\II\subseteq\LclRop{\Step[\JJ],\Step[\JJ]+\iSup{\JJ}}$
			\item $\Rwitness^i\Paren{\varphi_1,\varphi_2,\II}$
			\item $T_4\subseteq\Rproofset^i\Paren{\varphi_1,\varphi_2,\II,\JJ}$
			\end{myenums}
\end{myitems}
\end{multicols}
\end{pvstheorem}

One can use \aref{thm:until-witness-point} and \aref{thm:release-witness-interval} and follow the same steps explained in~\cite{96-MITL} to construct a \TAls\
for \aref{typ:nfUntil} and \aref{typ:nfRelease} formulas.
For example, if the automaton guesses $T_1$ is not empty then it must take this guess at time exactly $\iInf{T_1}$. At the same time, the automaton takes two 
more actions:
First,  it resets a {\em free} clock $x$ and remembers that this clock is not free anymore.
Second, it guesses whether $i$ should be $1$ or $2$. Suppose, $i$ is taken to be $1$.
As long as $x$ is not free, the automaton makes sure that the input signal satisfies $\varphi_1$.
Note that this is a different proof obligation and will be considered by an induction on the structure of input formula.
%
At the same time or at some time later, the automaton should guess $\iSup{T_1}$ is reached.
At any point in time, if the automaton does not make that call (\ie\ decides $\iSup{T_1}$ is not reached yet), it means the automaton wants to prove that 
the input signal satisfies the \UntilOp\ formula at all points in time between $\iInf{T_1}$ and sometime in the future.
%
As soon as the automaton guessed $\iSup{T_1}$ is reached, it resets a new free clock $y$ and marks it non-free.
%
The automaton then makes sure that when current values of $x$ and $y$ belong to $\II$, the input signal satisfies $\varphi_2$ at least once.
As soon as $\varphi_2$ becomes true during during this period, the proof obligation is over and $x$ and $y$ will both be marked as free clocks
(note that $\varphi_1$ does not need to be true when $\varphi_2$ becomes true).
%
Using \aref{thm:until-witness-point}, we know what the automaton checks, guarantees $\forall t\oftype T_1\WeHave f^t\NSat\Until{\varphi_1}{\varphi_2}[\II]$.
However, the automaton has only finitely many clocks and it cannot reuse a clock while it is not free.
The significance of \aref{thm:until-fv} is that it guarantees simultaneously guessing and proving at most $\Ceil{\frac{\iInf{\II}}{\Step[\II]}}+1$ number of 
$T_1$, $T_2$ intervals is enough. Since clocks $x$ and $y$ will be freed at most $\iSup{\II}$ units of time after they became non-free, number of required 
clocks for each \aref{typ:nfUntil} formula will be only twice the number of simultaneous proof obligations.
The same argument holds for \ReleaseOp\ operators, except that the automaton has to simultaneously guess and prove at most 
$\Ceil{\frac{\iInf{\II}}{\Step[\II]}}+1$ number of $T_1$, $T_2$, $T_3$, $T_4$ intervals.



==> part-related.tex <==
\section{Related Work}\label{sec:relateds}

Model checking and satisfiability of \MTL\ is proven to be undecidable in~\cite{96-MITL}.
The same paper introduces the first model checking and satisfiability algorithms for \MITL\ and \MITLzi, and proves optimality of them.
%
Different algorithms for model checking and satisfiability problems of \MITL\ formulas have been developed in the past.

In~\cite{06-MITL2TA}, authors introduce a different algorithm for transforming \MITL\ formulas into \TAlp.
In their work, two restrictions are enforced:
\begin{inparaenum}
\item they only support closed intervals in \MITL\ formulas, and
\item they only support signals that are continuous from right.
\end{inparaenum}
However, \aref{ex:2vars} and \aref{thm:2vars} in our paper, both use signals that are not continuous from right.
Therefore, their algorithm does not fix the problem in~\cite{96-MITL}.

Authors in~\cite{13-MITL2ATA,14-MITL2ATA} also consider transforming \MITL\ formulas into \TAlp, however they are using event-based semantics for \MITL\ 
formulas. In this semantics, one must specify time on which an event occurs. However, in state-based semantics that we used in our paper, such time might not 
exists. For instance, in \aref{ex:2vars}, atomic proposition $p$ is true during the interval $\Closed{0,c}$, but it is false for anytime after that.
Clearly, in this signal, there is not time in which $p$ is false for the first time.
 
Authors in~\cite{08-RecentMTL} nicely survey some recent results in \MTL.
They consider fragments of \MTL\ (including \LTL, \MITLzi, \MITL, \MTL, Bounded-\MTL, Safety-\MTL, and coFlat-\MTL), and review complexity of the corresponding 
model checking and satisfiability problems.

{\em Robust} model checking is a very important research area that deals with issues like noise in the environment, imprecise sensors, complexity, and 
implementability. However, robust model checking of \MTL\ formulas or its subclasses, has not been very active. To the best of our knowledge, 
\cite{08-robust-coFlatMTL} is the only paper in this area and considers robust model checking of coFlat-\MTL\ formulas.


